Input Prioritization for Testing Neural Networks

Deep neural networks (DNNs) are increasingly being adopted for sensing and control functions in a variety of safety and mission-critical systems such as self-driving cars, autonomous air vehicles, medical diagnostics, and industrial robotics. Failures of such systems can lead to loss of life or property, which necessitates stringent verification and validation for providing high assurance. Though formal verification approaches are being investigated, testing remains the primary technique for assessing the dependability of such systems. Due to the nature of the tasks handled by DNNs, the cost of obtaining test oracle data---the expected output, a.k.a. label, for a given input---is high, which significantly impacts the amount and quality of testing that can be performed. Thus, prioritizing input data for testing DNNs in meaningful ways to reduce the cost of labeling can go a long way in increasing testing efficacy. This paper proposes using gauges of the DNN's sentiment derived from the computation performed by the model, as a means to identify inputs that are likely to reveal weaknesses. We empirically assessed the efficacy of three such sentiment measures for prioritization---confidence, uncertainty, and surprise---and compare their effectiveness in terms of their fault-revealing capability and retraining effectiveness. The results indicate that sentiment measures can effectively flag inputs that expose unacceptable DNN behavior. For MNIST models, the average percentage of inputs correctly flagged ranged from 88% to 94.8%.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> ieee/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/2 <==

Motivation?
%
%In machine learning, having a large amount of training data is generally the
%key to achieving a high performance in a given
%task~\cite{havely2009unreasonable}.
%

When it comes to testing a trained model in the deployment environment, a
larger amount of test data may be required to assess how the model generalizes
to unseen data and perform as expected under diverse circumstances.
%
In such situations, collecting more data is less of a problem than obtaining
labeled data---the data that comes with both {\it input} and {\it expected
output}.
%
For example, consider a situation of testing an object detection model for
self-driving cars.
%
It may not be too difficult to simply collect more driving image data, 


Justification?

Introduce works from the SE subfield: {\it test prioritization for regression
testing}.

\subsection{Uncertainty-based Prioritization}


\subsection{Surprise-based Prioritization}

\subsection{Confidence-based Prioritization}



==> sections/motivation.tex <==
% sections/motivation.tex

%In machine learning, having a large amount of training data is generally the
%key to achieving a high performance in a given
%task~\cite{havely2009unreasonable}.

% What it means to test a model
In supervised learning, a model is learned from a given dataset where every
input is presented with a desired output called label~\cite{goodfellow2016deep}.
%
A learning algorithm such as stochastic gradient-descent~\cite{bottou2010large}
is used to optimize the model's parameter such that the cost measured by a
given cost function is minimized for the presented training dataset.
%
Since the input space that a model is expected to operate with is almost always
infinite, the challenge of supervised learning is to make sure that the model
performs well even with unseen data.
%
In practice, the performance of the trained model on {\it unseen data} is
estimated by testing the model with a set-aside validation dataset---a set of
labeled data that was intentionally held back from training the model.

This approach is premised on the assumption that the inputs used for
training and validation are truly representative of the actual inputs that
the DNN would encounter in its operational life, and that for the given
DNN, the validation data is adequate for determining that the DNN would 
generalize well to any new inputs that are in-distribution.
%
However, in practice, this will often not be the case for a variety of reasons.
%
The development may occur using a simulated environment for the system with
synthetic data which may not truly represent the actual input space that will be seen when the system is in operation.
%
Even if real operational data is used for training and validation, the data
distribution in the training and validation test sets may not be faithful
to the true distribution.
%
Finally, even if the test and validation data are truly representative,
there may be no easy way of determining that is indeed the case. 

One approach to addressing whether the DNN output should be trusted or not
on some previously unseen input data may to determine if the input is
in-distribution or out-of-distribution of the training and validation data,
Such a signal can be used as a way to determine when not to rely
on the DNN output.
%
However, even if the input is in-distribution, one 
may be still unsure if the training and validation data for the given 
DNN architecture sufficiently model the function to be realized.
\sanjai{do we need to look at work on determining out-of-distribution?}

Here, we take a complementary approach instead.
%
Rather than determining whether the
input is covered in the scope of the data that the DNN is trained on 
using a signal to indicate out-of-distribution, we look at whether 
the processing performed by the DNN on the input is in the scope of the
computations intended for the DNN, using a signal for sentiment.
This differentiation is somewhat akin to black-box versus white-box 
testing---both views are useful and likely complementary.
%
Inputs that indicate certain sentiments about the computation performed, such as low confidence,
high uncertainty or large surprise are considered to be stepping beyond the
scope of computations for which the DNN output can be trusted and thus
require further attention and intervention to label, retrain or simply
discard the output depending on the phase of the DNN development cycle.

We now briefly elaborate the need for this complementary approach.

\sanjai{if the above is acceptable then the following sections should be considerable shortened}.

\begin{comment}
\subsection{Model Validation is Not Enough}
% Validation testing is not enough.
Although it is tempting to extrapolate the validation accuracy as the test
accuracy, the generalization is bound by how well the validation dataset
represents the real input distribution, which is hard to know.
%
We demonstrate this fallacy with a small experiment, which shows a wide gap
between validation accuracy and test accuracy.
%
We designed four models of different structures and trained each of them with
MNIST dataset~\cite{lecun1998mnist}, a well-known dataset for hand-written
digit recognition task that is comprised of 70,000 data points; we used 60,000
data points for training and held out 10,000 for validation.
%
We fixed the batch size to 32, used ADAM optimizer~\cite{kingma2014adam},
check-pointed the epoch with the lowest validation loss, and stopped the
training when the validation loss did not improve for 20 consecutive epochs.
%
For testing the model with unseen data, we used EMNIST
dataset~\cite{cohen2017emnist}, which is another digit-recognition dataset that
consists of 280,000 data points designed to be compatible with MNIST.
\end{comment}



% Validation testing is not enough; more testing is necessary!
Table~\ref{tbl:generalization} shows the wide gap in the validation accuracy
and test accuracy.
%
While all of the four model achieved fairly high accuracies of $98.16\%$ to
$99.37\%$, the test accuracy varied dramatically from $77.39\%$ to $94.73\%$.
%
The result also shows that the validation accuracy alone can mislead us when
deciding which model is better.
%
Model C, for instance, achieved a higher validation accuracy than Model B,
while the test accuracy shows that Model B is better than Model C.
%
These mixed result suggests that validation testing alone is not a good-enough
measure of the real performance and that additional testing should be performed
comprehensively with more data in order to assess the generalization of the
trained model.


\begin{comment}

\subsection{Model Validation vs. User Validation}

\sanjai{This has to be shortened if at all it should be included}

From the perspective of Software Engineering, a program is verified against the
specification---to check if the program is {\it correct} with respect to how it
is designed---and validated against the requirement---to check if we developed
the {\it right} program that addresses the needs (of the
customers/users)~\cite{}.
%
Likewise, we argue that the learning-enabled component shall be verified and
validated in the same manner.
%
The difference, however, is that the traditional notion, mental framework,
techniques and tools may not directly portable to learning-enabled component
due to the distinct ways in which the learning-enabled components are
developed.
%
For instance, specification in a traditional sense translates {\it
"what"s}---the requirement---into {\it "how"s}~\cite{} so that the
implementation can be checked against the it.
%
For learning-enabled components, however, it is hard to refine the requirement
of the system into tangible {\it "how"s} since we rely on learning algorithms
to figure out the {\it "how"s} rather than coming up with rules to solve the
problem.
%
A digit classification task can be a good example; the requirement, although
vaguely, can be captured as "given an image of a digit between 0 and 9, assign
a correct label", while we cannot specify the {\it "how"} the system can
achieve it, any more clearly than "if it looks like 7, label it as 7. ...".


In the traditional software development life-cycle, testing activity could
address both of the two V\&V activities---verification was done by checking if
the program upholds the specification, and validation was done by checking if
the program meets the user requirement~\cite{}.
%
From this point of view, what is called validation testing in the deep learning
community is more like the verification in the traditional point of view when
we think of the training and validation data as capturing the specification
instance-by-instance.
%
This (model) validation testing is usually iterated multiple times while
adjusting the hyper-parameters to the model, just like the regression testing
is performed iteratively during development for checking the correctness of the
implementation.
%
The other testing---the testing for assessing the generalization of the
model---is much like the validation testing in a sense that it is performed
after the program is (almost) fully developed, and as it serves the purpose of
validating the program against the user requirement.
%
To avoid confusion with the term {\it validation testing} in the deep-learning
community, we call this process {\it user validation testing} and argue that
the main goal of user validation testing is to assess the generalization of the
model, and this is where we should focus our testing effort.
%
In the context of developing a deep-learning model, the user validation testing
would involve testing the generalization of the system with diverse range of
real inputs that are gathered from the operational environment.
%
The performance or the generalization of the model can then be analyzed and
{\it validated} against the system-level requirement.

\end{comment}


%This ability of the model to generalize to unseen data is informally called
%generalization, and we assume that the goal of testing should thusly focus on
%assessing the generalization of the model.

\subsection{Mitigating the Oracle Problem with Test Prioritization}


% It's hard to get labels
When it comes to testing for assessing generalization to large amount of unseen
data, the biggest bottleneck comes from labeling.
%
While it is relatively easy to obtain more test input, it is much more
difficult to obtain the expected output because the label cannot be created
automatically in most of the tasks that neural networks deal with.
%
For instance, consider a situation of testing an object detection model
designed for a self-driving car.
%
It is relatively cheap to collect more road image data, since a few vehicles
driven around the road can easily collect thousands of images every minute.
%
Labeling those images is much more expensive, however, since it inevitably
involves human effort of annotating the image with the objects recognized by
human.
%
If we assume that it takes 30 seconds for a person to label an image and the
frame rate of a camera is 30 FPS (frames per second), then it takes 15
man-hours for crafting the label for only an hour of driving data, which is
very costly ($3,600$ secs $\times$ $30$ FPS / $7,200$ images per hour).



% Oracle problem
From a software testing perspective, the difficulty of obtaining labeled data
is analogous to the difficulty of oracle construction known as the oracle
problem~\cite{barr2015oracle}.
%
However, due to characteristics unique to learning-enabled systems, many
of the solutions to the oracle problem studied by the software engineering
community cannot be applied directly.
%
For instance, one of the most straight-forward and natural way of producing an
oracle is to harness the specification, which is an artifact that specifies the
behavior of a software.
%
When available, formal or informal specification, state transition system,
assertions, and contracts can directly or indirectly be used to construct test
oracles.
%
We cannot obtain this type of oracle for most of the tasks that machine
learning deals with.
%
Object detection is one of such problem of perception---it is not possible to
unambiguously specify what an object looks like, let alone creating an
automated oracle.



% How we solve the problem
This work attempts to tackle the oracle problem by reducing the cost of
labeling.
%
First, we assume that not every test input is of the same value.
%
For the most practical goal of testing is to find as many bugs as possible, an
input that reveals a misbehavior of the model is more valuable than an input
that does not.
%
Second, we hypothesize that the relative value of each test input---or the
likelihood of each input of triggering a erroneous behavior---can be
automatically estimated by a systematic measure.
%
We introduce three measures of uncertainty based on white-box analysis of the
neural network which can assign relative value of utility to the unlabeled test
input.

\begin{comment}
If these assumptions hold, we can reduce the cost of neural network testing
dramatically, by having to label only a fraction of the test inputs that are
most likely to reveal faults.
%
For instance, one can run a million test inputs and get a similar amount of
insight, or catch a similar number of bugs only by inspecting a thousand inputs
manually instead of a million.
\end{comment}



==> sections/uncertainty_adequacy.tex <==


Void


==> tables/tbl_mcdc.tex <==
\renewcommand{\arraystretch}{1.0}
\setlength\tabcolsep{4pt}
\begin{tabular}{lrrrrrr}
%\hline
\toprule
%\small
\multirow{2}{*}{{Case Example}} & \multicolumn{2}{c}{MC/DC}
    & \multicolumn{2}{c}{Flag-Use OBC} & \multicolumn{2}{c}{OBC} \\%\cline{2-7}
\cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}
& \multicolumn{1}{c}{mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{mean}
& \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{mean} & \multicolumn{1}{c}{SD} \\
%\cmidrule(r){1-1}\cmidrule(r){2-2}\cmidrule(r){3-3}\cmidrule(r){4-4}\cmidrule(r){5-5}\cmidrule(r){6-6}\cmidrule(r){7-7}
\midrule
Microwave (C) & 64.95 & 2.49 & 63.57 & 3.35 & 63.19 & 3.60 \\ %\hline
Microwave & 65.59 & 3.11 & 54.67 & 5.37 & 45.38 & 10.91 \\ %\hline
Infusion Pump & 15.51 & 1.99 & 13.17 & 1.95 & 11.34 & 2.61 \\ %\hline
Docking Approach & 17.32 & 2.36 & 20.70 & 1.36 & 18.93 & 2.76 \\ %\hline
Cruise Controller & 3.48 & 1.09 & 4.11 & 1.31 & 3.29 & 1.79 \\ %\hline
\bottomrule
\end{tabular}

\begin{comment}
\setlength\tabcolsep{3pt}
\begin{tabular}{|l||r|r|r|r|r|r|}
\hline
%\small
\multirow{2}{*}{System} & \multicolumn{2}{c|}{MC/DC}
    & \multicolumn{2}{c|}{Flag-Use OBC} & \multicolumn{2}{c|}{OBC}
\\\cline{2-7}
& mean & SD & mean & SD & mean & SD \\ \hline
Microwave (C) & 64.95 & 2.49 & 63.57 & 3.35 & 63.19 & 3.60 \\ \hline
Microwave & 65.59 & 3.11 & 54.67 & 5.37 & 45.38 & 10.91 \\ \hline
Infusion Pump & 15.51 & 1.99 & 13.17 & 1.95 & 11.34 & 2.61 \\ \hline
Docking Approach & 17.32 & 2.36 & 20.70 & 1.36 & 18.93 & 2.76 \\ \hline
Cruise Controller & 3.48 & 1.09 & 4.11 & 1.31 & 3.29 & 1.79 \\ \hline
\end{tabular}
\end{comment}

